Detecting and Understanding the Promotion of Illicit Goods and Services on Twitter

In this study, we reveal, for the first time, popular online social networks (especially Twitter) are being extensively abused by miscreants to promote illicit goods and services of diverse categories. This study is made possible by multiple machine learning tools that are designed to detect and analyze Posts of Illicit Promotion (PIPs) as well as revealing their underlying promotion campaigns. Particularly, we observe that PIPs are prevalent on Twitter, along with extensive visibility on other three popular OSNs including YouTube, Facebook, and TikTok. For instance, applying our PIP hunter to the Twitter platform for 6 months has led to the discovery of 12 million distinct PIPs which are widely distributed in 5 major natural languages and 10 illicit categories, e.g., drugs, data leakage, gambling, and weapon sales. Along the discovery of PIPs are 580K Twitter accounts publishing PIPs as well as 37K distinct instant messaging accounts that are embedded in PIPs and serve as next hops of communication with prospective customers. Also, an arms race between Twitter and illicit promotion operators is also observed. Especially, 90% PIPs can survice the first two months since getting published on Twitter, which is likely due to the diverse evasion tactics adopted by miscreants to masquerade PIPs.

==> 8_conclusion.tex <==
Through this study, we have qualified and quantified the prevalence of diverse posts of illicit promotions (PIPs) on Twitter. Also, it is observed that illicit operators have adopted various evasion tactics when composing and distributing PIPs, which partially explains why so many PIPs could circumvent the content moderation of Twitter, get posted, and keep alive for months before being unpublished. What is also observed is that accounts of instant messaging platforms, especially end-to-end encrypted ones, are frequently used as the next hops for the communication between PIP victims and the underlying illicit operators. Such a cross-platform operation pattern 
also highlights the importance of security collaborations among OSN and instant messaging platforms for the mitigation of illicit promotion activities. 
